Uniform hyperbolicity of the curve graph via surgery sequences

We prove that the curve graph $\calC^{(1)}(S)$ is Gromov-hyperbolic with a constant of hyperbolicity independent of the surface $S$. The proof is based on the proof of hyperbolicity of the free splitting complex by Handel and Mosher, as interpreted by Hilion and Horbez.

==> header_article.tex <==
%%% Environments %%%

% Numbering
% see http://tex.stackexchange.com/questions/41299/how-to-identify-the-counter-of-equation-theorem-and-section

\makeatletter
\let\c@equation\c@subsection
\makeatother
\numberwithin{equation}{section} 

\makeatletter
\let\c@figure\c@equation
\makeatother
\numberwithin{figure}{section} 

% Formatting 
% see amsthdoc.pdf for general discussion. 

\theoremstyle{plain}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{principle}[equation]{Principle}
\newtheorem{axiom}[equation]{Axiom}

\theoremstyle{definition}
\newtheorem{definition}[equation]{Definition}
\newtheorem{problem}[equation]{Problem}
\newtheorem{solution}[equation]{Solution}
\newtheorem{exercise}[equation]{Exercise}
\newtheorem{example}[equation]{Example}
\newtheorem{fact}[equation]{Fact}
\newtheorem{question}[equation]{Question}
\newtheorem*{question*}{Question}
\newtheorem*{answer*}{Answer}
\newtheorem*{application*}{Application}
\newtheorem{algorithm}[equation]{Algorithm}
\newtheorem{objective}{Objective}[section]

\theoremstyle{remark}
\newtheorem{remark}[equation]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{remarks}[equation]{Remarks}
\newtheorem{case}{Case}
\newtheorem*{case*}{Case}
\newtheorem*{step*}{Step}
%\renewcommand{\thecase}{\Roman{case}}
\newtheorem{claim}[equation]{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem*{proofclaim}{Claim}
\newtheorem*{proofsubclaim}{Subclaim}

%%% Refs
\newcommand{\refsec}[1]{Section~\ref{Sec:#1}}
\newcommand{\refapp}[1]{Appendix~\ref{App:#1}}
\newcommand{\refthm}[1]{Theorem~\ref{Thm:#1}}
\newcommand{\refcor}[1]{Corollary~\ref{Cor:#1}}
\newcommand{\reflem}[1]{Lemma~\ref{Lem:#1}}
\newcommand{\refprop}[1]{Proposition~\ref{Prop:#1}}
\newcommand{\refclm}[1]{Claim~\ref{Clm:#1}}
\newcommand{\refrem}[1]{Remark~\ref{Rem:#1}}
\newcommand{\refexa}[1]{Example~\ref{Exa:#1}}
\newcommand{\reffac}[1]{Fact~\ref{Fac:#1}}
\newcommand{\refexe}[1]{Exercise~\ref{Exe:#1}}
\newcommand{\reffig}[1]{Figure~\ref{Fig:#1}}
\newcommand{\refdef}[1]{Definition~\ref{Def:#1}}
\newcommand{\refprob}[1]{Problem~\ref{Prob:#1}}
\newcommand{\refalg}[1]{Algorithm~\ref{Alg:#1}}
\newcommand{\refax}[1]{Axiom~\ref{Ax:#1}}
\newcommand{\refeqn}[1]{Equation~\ref{Eqn:#1}}
\newcommand{\refconj}[1]{Conjecture~\ref{Conj:#1}}
\newcommand{\refobj}[1]{Objective~\ref{Obj:#1}}

